Just Weather Scoring: Efficient End-to-end Nowcasting with Distributional Diffusion

Generative diffusion models are well-suited for probabilistic precipitation nowcasting, but existing approaches often rely on separately trained compression or deterministic forecasting components and remain costly at inference due to iterative denoising. We introduce Just Weather Scoring (JWS), a single-stage, end-to-end diffusion model which addresses both issues by forecasting directly in radar space and enabling few-step generation. Radar-space modeling greatly simplifies training and inference and eliminates uncertainty arising from lossy compression. JWS combines Masked Asynchronous Diffusion, a timestep-sampling scheme that preserves clean context while adapting diffusion training to high-dimensional spatio-temporal data, with a simple scoring-rule objective that aligns training with probabilistic forecasting and unlocks few-step generation. On the SEVIR and MeteoNet benchmarks, JWS achieves state-of-the-art probabilistic forecasting performance at reduced training and inference cost. Even our smallest model remains competitive using substantially fewer parameters and more than 17x faster inference.

==> figs/4_exp/ablations_t_sample_paradigm_sampler.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.31\textwidth}
        \includegraphics[width=\textwidth]{figs/tmp/t_sampling_ramvid.png}
        \caption{T-sampling.}\label{fig:exp:ablations:t_sampling}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.31\textwidth}
        \includegraphics[width=\textwidth]{figs/tmp/paradigm_over_training.png}
        \caption{Paradigm.}\label{fig:exp:ablations:paradigm}
    \end{subfigure}
    \caption{\textbf{T-sampling Paradigm.} \todo{t-sampling from JiT does not work, RaMViD Forcing is stable, strong, and flexible; stochastic samplers bring additional benefits, distributional training enables new sampling schemes}}
    \label{fig:exp:ablations}
\end{figure}

==> figs/4_exp/rank_histogram.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\textwidth]{figs/4_exp/plots/rank_histogram.pdf}
        \caption{Time-averaged.}\label{fig:exp:rank_histogram:mean}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\textwidth]{figs/4_exp/plots/reliability_index_over_time.pdf}
        \caption{RI over lead time.}\label{fig:exp:rank_histogram:ri_over_t}
    \end{subfigure}
    \hfill
    % \begin{subfigure}{0.32\textwidth}
    %     \includegraphics[width=\textwidth]{figs/4_exp/plots/rank_histogram_t11.pdf}
    %     \caption{$+60$\,min.}\label{fig:exp:rank_histogram:last_t}
    % \end{subfigure}
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\textwidth]{figs/4_exp/plots/ablation_detcond_nfe_ri.pdf}
        \caption{Deterministic Prior.}\label{fig:exp:rank_histogram:ri_detcond}
    \end{subfigure}
    \caption{\textbf{Calibration.} \ours~produces a flatter rank histogram and remains better calibrated for the entire lead time range. Conditioning generation on a deterministic prior deteriorates calibration.}\label{fig:exp:rank_histogram}
\end{figure}

==> figs/4_exp/sevir_objective_nfe.tex <==
% \begin{figure}
%     \centering
%     \begin{subfigure}{\textwidth}
%         \includegraphics[width=\linewidth]{figs/4_exp/plots/ablation_objective_nfe.pdf}
%     \end{subfigure}
%     \par\vspace{0.3cm}
%     \begin{subfigure}{\textwidth}
%         \includegraphics[width=\linewidth]{figs/4_exp/plots/ablation_ddm_nfe.pdf}
%     \end{subfigure}    
%     \caption{\textbf{Distributional Training Objective.} Training with a distributional objective unlocks few-step inference. However, using only CRPS or a DDM objective diverges for high NFE. Both iDDM and sDD remain stable for low and high NFE. Yet, our sDD objective achieves consistently superior performance. Ablation done with S-scale model using 512 samples.}
%     \label{fig:exp:objective}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/4_exp/plots/ablation_objective_iddm_nfe_bars.pdf}
    \caption{\textbf{Distributional Training Objective.} Training with a distributional objective unlocks few-step inference. However, using only the distributional loss diverges for high NFE.}
    \label{fig:exp:objective}
\end{figure}

==> figs/4_exp/sevir_qualitative.tex <==
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{0.1pt}
    \newcommand{\imagesize}{0.1\textwidth}
    \newcommand{\imgpath}{figs/4_exp/qualitative_comparison/idx2289}
    \newcommand{\gridimage}[3]{\includegraphics[width=\imagesize]{\imgpath/#1_#2_#3.png}}
    \newcommand{\rowlabel}[1]{%
        \raisebox{%
            \dimexpr\imagesize/2-\height/2+\depth/2\relax
        }[0pt][0pt]{%
            \rotatebox{90}{#1}%
        }%
    }
    \begin{tabular}{ccccccc}
        & +10\,min & +20\,min & +30\,min
        & +40\,min & +50\,min & +60\,min \\
    
        % \rowlabel{\footnotesize CasCast}
        % & \gridimage{cascast}{2}{1}
        % & \gridimage{cascast}{4}{1}
        % & \gridimage{cascast}{6}{1}
        % & \gridimage{cascast}{8}{1}
        % & \gridimage{cascast}{10}{1}
        % & \gridimage{cascast}{12}{1} \\
    
        \rowlabel{\footnotesize FREUD}
        & \gridimage{freud}{2}{1}
        & \gridimage{freud}{4}{1}
        & \gridimage{freud}{6}{1}
        & \gridimage{freud}{8}{1}
        & \gridimage{freud}{10}{1}
        & \gridimage{freud}{12}{1} \\
    
        \rowlabel{\footnotesize JWS {\tiny (Ours)}}
        & \gridimage{ours}{2}{1}
        & \gridimage{ours}{4}{1}
        & \gridimage{ours}{6}{1}
        & \gridimage{ours}{8}{1}
        & \gridimage{ours}{10}{1}
        & \gridimage{ours}{10}{1} \\
    
        \rowlabel{\footnotesize GT}
        & \gridimage{gt}{2}{1}
        & \gridimage{gt}{4}{1}
        & \gridimage{gt}{6}{1}
        & \gridimage{gt}{8}{1}
        & \gridimage{gt}{10}{1}
        & \gridimage{gt}{12}{1}
    \end{tabular}
    \caption{\textbf{Qualitative Forecast Comparison.} \ours~produces forecasts that are better aligned with the ground truth than CasCast and FREUD predictions.\jannik{show map}}
    \label{fig:exp:qualitative_comp}
\end{figure}

==> figs/4_exp/sevir_qualitative_ensemble.tex <==
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{0.1pt}
    \newcommand{\imagesize}{0.1\textwidth}
    \newcommand{\imgpath}{figs/4_exp/qualitative_ensemble/}
    \newcommand{\gridimage}[4]{\includegraphics[width=\imagesize]{\imgpath/idx#1/#2_#3_#4.png}}
    \newcommand{\gridimagerow}[1]{\gridimage{#1}{gt}{12}{1} & \gridimage{#1}{ens}{12}{1} & \gridimage{#1}{ens}{12}{2} & \gridimage{#1}{ens}{12}{3} & \gridimage{#1}{ens}{12}{4} & \gridimage{#1}{ens}{12}{5} & \gridimage{#1}{var}{12}{1} & \colorbar{#1}{12} \\}
    \newcommand{\colorbar}[2]{\includegraphics[height=0.1\textwidth]{\imgpath/idx#1/colorbar_#2.pdf}}
    \begin{tabular}{cccccccc}
        GT & Ens 1 & Ens 2 & Ens 3 & Ens 4 & Ens 5 & Var & \\
        \gridimagerow{1679}
        \gridimagerow{2286}
        % \gridimagerow{12149}
    \end{tabular}
    \caption{\textbf{Qualitative Forecast Ensemble.} At $+60\,\text{min}$ \ours~still produces ensemble members with similar global structure, while showing variability in chaotic local details. Ensemble variance is aligned with precipitation intensity, matching expected predictability structure.\joh{show map}}
    \label{fig:exp:qualitative_ens}
\end{figure}

==> figs/4_exp/sevir_scaling.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\textwidth]{figs/tmp/model_size_train_steps.png}
        \caption{Model Size}\label{fig:exp:scaling:model}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\textwidth]{figs/tmp/patch_size_over_training.png}
        \caption{Patch size / number of tokens}\label{fig:exp:scaling:patch}
    \end{subfigure}
    \caption{\textbf{Model Scaling} \todo{we can scale the model along the number of parameters of number of tokens (patch size) consistently} \jannik{It would be super cool to also show data scaling but I don't think that is feasible at the moment}}
    \label{fig:exp:scaling}
\end{figure}

==> figs/4_exp/sevir_test_scaling.tex <==
% \begin{figure}
%     \centering
%     \begin{subfigure}{0.31\textwidth}
%         \includegraphics[width=\linewidth]{figs/tmp/model_scale_NFE.png}
%         \caption{NFE.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.31\textwidth}
%         \includegraphics[width=\linewidth]{figs/tmp/model_size_ensemble.png}
%         \caption{Ensemble Size.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figs/tmp/ensemble_scaling.png}
%         \caption{Mode Collapse.}\label{fig:exp:test_time_scaling:ensemble}
%     \end{subfigure}
%     \caption{\textbf{Test-time scalability.} \todo{Our model is highly efficient enabling using more NFE and ensemble members and scales consistently when investing compute into either}}
%     \label{fig:exp:test_time_scaling}
% \end{figure}

==> figs/radar-noise-schedules/figure.tex <==
\begin{figure}[htbp]
    \centering
    \setlength{\tabcolsep}{1pt}
    \scriptsize
    \newcommand{\radarschedulemap}[2]{%
        \includegraphics[width=0.075\linewidth]{figs/radar-noise-schedules/radar-384x384-#1-t#2.png}%
    }
    \begin{tabular}{@{}l*{11}{c}@{}}
        $\tilde{\tau}$ & $0.0$ & $0.1$ & $0.2$ & $0.3$ & $0.4$ & $0.5$
        & $0.6$ & $0.7$ & $0.8$ & $0.9$ & $1.0$ \\
        \raisebox{0.023\linewidth}{Unshifted}
        & \radarschedulemap{unshifted}{0.0}
        & \radarschedulemap{unshifted}{0.1}
        & \radarschedulemap{unshifted}{0.2}
        & \radarschedulemap{unshifted}{0.3}
        & \radarschedulemap{unshifted}{0.4}
        & \radarschedulemap{unshifted}{0.5}
        & \radarschedulemap{unshifted}{0.6}
        & \radarschedulemap{unshifted}{0.7}
        & \radarschedulemap{unshifted}{0.8}
        & \radarschedulemap{unshifted}{0.9}
        & \radarschedulemap{unshifted}{1.0} \\
        \raisebox{0.023\linewidth}{\shortstack[l]{Spatial\\shift}}
        & \radarschedulemap{spatial-shift}{0.0}
        & \radarschedulemap{spatial-shift}{0.1}
        & \radarschedulemap{spatial-shift}{0.2}
        & \radarschedulemap{spatial-shift}{0.3}
        & \radarschedulemap{spatial-shift}{0.4}
        & \radarschedulemap{spatial-shift}{0.5}
        & \radarschedulemap{spatial-shift}{0.6}
        & \radarschedulemap{spatial-shift}{0.7}
        & \radarschedulemap{spatial-shift}{0.8}
        & \radarschedulemap{spatial-shift}{0.9}
        & \radarschedulemap{spatial-shift}{1.0} \\
        \raisebox{0.018\linewidth}{\shortstack[l]{Spatial +\\temporal\\shift}}
        & \radarschedulemap{thw-shift}{0.0}
        & \radarschedulemap{thw-shift}{0.1}
        & \radarschedulemap{thw-shift}{0.2}
        & \radarschedulemap{thw-shift}{0.3}
        & \radarschedulemap{thw-shift}{0.4}
        & \radarschedulemap{thw-shift}{0.5}
        & \radarschedulemap{thw-shift}{0.6}
        & \radarschedulemap{thw-shift}{0.7}
        & \radarschedulemap{thw-shift}{0.8}
        & \radarschedulemap{thw-shift}{0.9}
        & \radarschedulemap{thw-shift}{1.0} \\
    \end{tabular}
    \caption{\textbf{Dimensionality-aware corruption of a SEVIR radar map.}
    All panels have resolution $384\times384$. Columns show pre-shift diffusion times $\tilde{\tau}$.
    Rows show unshifted interpolation ($\tau=\tilde{\tau}$), spatial shifting ($D=384^2$), and
    spatio-temporal shifting ($D=25\cdot384^2$). Both shifts follow
    \cref{eq:spatiotemporal_timestep_shift} with reference dimensionality $D_0=256^2$.
    The same radar frame and Gaussian noise realization are used throughout, with
    $\mathbf{x}_{\tau}=(1-\tau)\boldsymbol{\epsilon}+\tau\mathbf{x}_1$;
    $\tau=0$ denotes noise and $\tau=1$ clean radar data.
    Radar values are normalized to $[-1,1]$ before interpolation, and all panels use the same color scale. \joh{double check caption etc}}
    \label{fig:radar-noise-schedules}
\end{figure}

